One word at a time: adversarial attacks on retrieval models

Adversarial examples, generated by applying small perturbations to input features, are widely used to fool classifiers and measure their robustness to noisy inputs. However, little work has been done to evaluate the robustness of ranking models through adversarial examples. In this work, we present a systematic approach of leveraging adversarial examples to measure the robustness of popular ranking models. We explore a simple method to generate adversarial examples that forces a ranker to incorrectly rank the documents. Using this approach, we analyze the robustness of various ranking models and the quality of perturbations generated by the adversarial attacker across two datasets. Our findings suggest that with very few token changes (1-3), the attacker can yield semantically similar perturbed documents that can fool different rankers into changing a document's score, lowering its rank by several positions.

==> Adversarial Attack on Rankers/src/abstract.tex <==
Adversarial examples, generated by applying small perturbations to input features, are widely used to fool classifiers and measure their robustness to noisy inputs. However, little work has been done to evaluate the robustness of ranking models through adversarial examples.
In this work, we present a systematic approach of leveraging adversarial examples to measure the robustness of popular ranking models. We explore a simple method to generate adversarial examples that forces a ranker to incorrectly rank the documents. Using this approach, we analyze the robustness of various ranking models and the quality of perturbations generated by the adversarial attacker across two datasets. Our findings suggest that with very few token changes (1-3), the attacker can yield semantically similar perturbed documents that can fool different rankers into changing a document's score, lowering its rank by several positions. 


==> Adversarial Attack on Rankers/src/approach.tex <==
\section{Our Approach}
\label{sec:approach}
Our goal is to minimally perturb a document such that the rank of the document changes. 
In particular, we target top-ranked documents and attempt to lower their rank through noise
injection. Assuming relevant documents are ranked higher, the objective is to lower the position of a document with minimal change in its text.
\subsection{Problem Statement}
Let $\Vec{q}$, $\Vec{d}$ and $\mathcal{F}$ represent a query, a document and a ranking model, respectively.
Given a query-document pair $(\Vec{q},\Vec{d})$, the ranker outputs a score $s=\mathcal{F}(\Vec{q},\Vec{d})$ indicating
the relevance of the document $\Vec{d}$ to the query $\Vec{q}$, where higher score means higher relevance.
Given a query and a list of documents, the ranker computes scores for every document w.r.t the 
given query and rank documents based on a descending order of the scores.
Given $\Vec{q}$ and $\Vec{d}$, our goal is to find a perturbed document $\Vec{d'}$ such that 
$\mathcal{F}(\Vec{q},\Vec{d'}) << \mathcal{F}(\Vec{q},\Vec{d})$ so that it ranks lower than
its original rank. At the same time we want to minimize the perturbation in the document.
%otherwise perturbed text can be very noisy and non-relevant with respect to the query.

We assume that both query and document are represented as vectors which could be either sequence of
terms or other suitable representations such as word embedding. Let $\Vec{q} = (q_1, q_2, ..., q_p)$
be a p-dimensional query vector and $\Vec{d} = (d_1, d_2, ..., d_q)$ be a q-dimensional document
vector. We construct a perturbed document $\Vec{d'}=(\Vec{d} + \Vec{n})$ by adding a q-dimensional noise vector 
$\Vec{n} = (n_1, n_2, ..., n_q)$. 
Our goal is to find a noise vector that reduces a document's score
without changing many terms in the document. 
% The noise vector should satisfy the following properties:
% 1) it should reduce the document's score, 
% 2) it should be sparse (should not change many terms in the document), and
% 3) it should not change the document significantly.
We formulate this problem as an optimization problem as follows:
\begin{equation}
\label{eq:v1}
\begin{aligned}
& \underset{\Vec{n}}{\text{minimize}}
& & \mathcal{F}(\Vec{q}, \Vec{d+n}) \\
& \text{subject to}
& & ||\Vec{n}||_0 \leq c 
\end{aligned}
\end{equation}
Here, $c$ is a sparsity parameter that controls the number of perturbed terms.
Although, the above formulation provides a sparse solution, we do not have
any control over the magnitude of the noise vector. In other words,
even though we change only few terms in a document we may end up
changing them significantly. To address this problem, we modify the 
objective function as follows:
\begin{equation}
\label{eq:v2}
\begin{aligned}
& \underset{\Vec{n}}{\text{minimize}}
& & \mathcal{F}(\Vec{q}, \Vec{d+n}) + \sum_{i=1}^{q}{\mathcal{D}}(d_i, (d_i+n_i)) \\
& \text{subject to}
& & ||\Vec{n}||_0 \leq c 
\end{aligned}
\end{equation}
Here, $\mathcal{D}$ can be any suitable distance function (e.g., cosine distance)
that computes distance between two terms. 
It ensures that the modified terms are close to the original terms.
We found this formulation too strict. 
In particular, it penalizes perturbations of query terms as well non-query
terms in a document. Hence, we modify the objective function to penalize
only query terms since we want to ensure that the perturbed document
stays relevant to the query. The modified objective function is as follows:
\begin{equation}
\label{eq:v3}
\begin{aligned}
& \underset{\Vec{n}}{\text{minimize}}
& & \mathcal{F}(\Vec{q}, \Vec{d+n}) + \sum_{i=1}^{q} \mathbbm{1}_{d_i \in \Vec{q}} [{\mathcal{D}}(d_i, (d_i+n_i))] \\
& \text{subject to}
& & ||\Vec{n}||_0 \leq c 
\end{aligned}
\end{equation}
Here, $\mathbbm{1}_{x}$ is an indicator function with is $1$ when $x$ is true and $0$ otherwise.
The first term in the objective function ensures that the ranker gives low score to the perturbed document
while the second term incurs penalty of changing query terms in the document. 
The constrains limits the number of changed terms in a document to $c$.

\subsection{Method}
A popular approach to solve the above problem relies on computing gradient of the model's output (score) with respect to the input and use this gradient to find a noise vector that reduces model's score on noisy input~\cite{fgsm}.
Such gradient based methods do not work well with textual data due to non-differentiable components 
such as an embedding layer. 
A common workaround is to find perturbation in the embedding space and project the perturbation vector in the input space
through techniques like nearest neighbour search. In general, gradient based methods are restricted to differentiable models and require information about the model's architecture.

To address the shortcomings of gradient based methods, we propose a different approach that uses Differential Evolution (DE)~\cite{de}, a stochastic evolutionary algorithm. It can be applied to a variety of optimization problems including non-differentiable and multimodal objective functions. DE is a population-based optimization method which works as follows:
Let's say we want to optimize over $l$ parameters. Given the population size $m$, it randomly initializes $m$ candidate solutions $\Vec{X_t} = (\Vec{x}_1, \Vec{x}_2, ..., \Vec{x}_m)$, each of length $l$. From these parent solutions it generates candidate children solutions using the following mutation criteria: 
\begin{equation}
    \Vec{x}_{a,t+1} = \Vec{x}_{b,t} + F(\Vec{x}_{c,t} - \Vec{x}_{d,t})
    % \; \; \; \; (a \neq b \neq c \neq d)
\end{equation}

Here, $a, b, c$ and $d$ are randomly chosen distinct indices in the population, and $F$ is a mutation factor in $[0,2]$. Next, these children are compared against their parents using a fitness function and $m$ candidates are selected that have the highest fitness (i.e., minimizes the fitness function). This process is repeated until either it converges or reaches the maximum number of iterations.

Given a query-document pair $(\Vec{q},\Vec{d})$ and a trained ranker $\mathcal{F}$ we use DE to find a perturbation vector $\Vec{n}$ 
that changes the document's rank without significantly modifying it.
In particular, we need to find what terms to perturb in the document and the magnitude of each perturbation. Hence, we represent the solution (perturbation vector) as a sequence of tuples $(i, v)$ where $i \in [0,|\Vec{d}|]$ represents an index of the term to perturb and $v$ represents the perturbation value. The length of the solution vector is set to $c$ (the sparsity parameter). 
We use the objective function proposed earlier as a fitness function for DE and run the algorithm for a fixed number of iterations.
Based on the choice of the fitness function, we propose three variants of the attack, \vone (Equation~\ref{eq:v1}), \vtwo (Equation~\ref{eq:v2}) and \vthree (Equation~\ref{eq:v3}). 
The final solution vector is used to construct the perturbed document $d'$. A similar approach has been used to perturb images in order to fool a classifier~\cite{onepixel}.






==> Adversarial Attack on Rankers/src/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
Adversarial attacks on classification models both in text and vision have helped reduce the generalization error of such models. However, there is limited literature on adversarial attacks on information retrieval models. In this work, we explored effectiveness and quality of three simple methods of attacking black box deep learning models. The attackers were designed to change document text such that an information retrieval model is fooled into lowering the document position. We found that perturbed text generated by these attackers by changing few tokens is semantically similar to original text and \emph{can fool} the ranker to push a relevant document below $\sim$2-3 non-relevant documents. Our findings can be further used to train rankers with adversarial examples to reduce their generalization error. 


==> Adversarial Attack on Rankers/src/experiments.tex <==

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}\hline
\textbf{Dataset} & \textbf{Model} & \textbf{\sk} & \vzero & \vone & \vtwo & \vthree  \\ \hline
\multirowcell{6}{WikiQA\\} & \multirowcell{2}{DRMM\\} & 1 & 0.62 & 1.0 & 0.93 & 1.0 \\  
                                                    & & 5 & 0.01 & 0.26 & 0 & 0.15 \\  \cline{2-7}
                           & \multirowcell{2}{Duet\\} & 1 & 0.58 & 1.0 & 0.65 & 1.0 \\  
                                                    & & 5 & 0.02 & 0.27 & 0 & 0.25 \\  \cline{2-7}
                           & \multirowcell{2}{KNRM\\} & 1 & 0.56 & 1.0 & 0.41 & 1.0 \\  
                                                    & & 5 & 0 & 0.13 & 0.01 & 0.13 \\  \hline
\multirowcell{6}{MSMarco\\} & \multirowcell{2}{DRMM\\} & 1 & 0.67 & 1.0 & 0.73 & 1.0 \\  
                                                    & & 5 & 0 & 0.11 & 0.003 & 0.04 \\  \cline{2-7}
                           & \multirowcell{2}{Duet\\} & 1 & 0.5 & 1.0 & 0.57 & 1.0 \\  
                                                    & & 5 & 0 & 0.87 & 0.03 & 0.81 \\  \cline{2-7}
                           & \multirowcell{2}{KNRM\\} & 1 & 0.58 & 1.0 & 0.89 & 1.0 \\  
                                                    & & 5 & 0.01 & 0.89 &0.45 & 0.89 \\  \hline
    \end{tabular}
    \caption{Attackers' success on changing document's position.}
    \label{table:success}
\end{table}
\section{Experimental Setup}
\label{sec:experiments}
%We evaluate the proposed adversarial attacks on three ranking models.
In this section, we provide details about the datasets, model training, perturbation and evaluation metrics. \newline
\textbf{Data:} We use WikiQA~\cite{wikiqa} and MSMarco passage ranking dataset~\cite{msmarco} for training ranking models and evaluating attacks on three ranking models.
For WikiQA, we use 2K queries for training and 240 queries for evaluation.
For MSMarco, we use 20K randomly sampled queries for training and 220 queries for evaluation. 
For each test query, we randomly sample 5 positive documents and 45 negative documents for evaluation. \newline
\textbf{Model training:} We use the following ranking models: 
DRMM~\cite{drmm}, DUET~\cite{duet} and KNRM~\cite{knrm}.
We use 300 dimensional Glove embeddings~\cite{glove} to represent each token. \newline
%All models are trained using MatchZoo\footnote{https://github.com/NTMC-Community/MatchZoo} library. \newline
\textbf{Perturbation:}
In our experiments, we perturb \emph{only} relevant documents\footnote{We found that non-relevant documents can be perturbed easily by adding noisy text.} in top 5 results for each query in the test set. 
We perturb documents using all three attackers (\vone, \vtwo, and \vthree) and evaluate ranker performance on the perturbed documents. 
The number of iterations and population size are fixed to 100 and 500 respectively. \newline
\textbf{Evaluation:}
We explore several metrics for understanding the effectiveness of perturbations and their impact on ranker performance. The goal of an   attacker is to fool the ranker into lowering the position of the document in the list. The success of the attacker is measured as the percentage of \emph{relevant} documents whose position changed by $k$ when perturbed by the attacker. Let $\mathcal{R}(d)$ denote the rank of a document $d$ and $l_d$ denote its relevance. Then, the attacker's success at k (\sk) is defined as follows:
\begin{equation*}
    \sk = \frac{\sum_{d; l_d>0} \mathbbm{1}_{(\mathcal{R}(d') - \mathcal{R}(d)) >= k}}{\sum_{d; l_d>0} \mathbbm{1}}
\end{equation*}

Here, $d'$ is a perturbation of $d$ generated by the attacker. 
We also measure the number of non-relevant documents crossed (\nrc) by perturbing $d$ to $d'$ as defined below:
\begin{equation*}
    \nrc = \sum_{\hat{d}; l_{\hat{d}}=0} \mathbbm{1}_{\mathcal{R}(d) < \mathcal{R}(\hat{d}) < \mathcal{R}(d')}
\end{equation*}
% \mathcal{R}(d) < \mathcal{R}(\hat{d}) < \mathcal{R}(d')
%Apart from these, we explore several other metrics for understanding the quality of perturbations and their impact on ranker performance.
We compare the performance of the proposed attacks against a random baseline \vzero where the adversary perturbs a word at random from the text and replaces it with the most similar word (minimum cosine distance in the embedding space) from the corpus.


\begin{table}[t]
    \centering
    \begin{tabular}{|c|c |c|c |c| }\hline
\textbf{Model} & \textbf{Atk}  & 1 token & 3 tokens & 5 tokens  \\ \hline
\multirowcell{3}{DRMM\\} &\vone&  0.944$\pm$2.776	&	3.867$\pm$6.334	&	6.814$\pm$7.858\\  
&\vtwo&  0.037$\pm$0.623	&	0.304$\pm$1.752	&	0.647$\pm$3.129\\
&\vthree&0.404$\pm$1.730	&	1.280$\pm$3.388	&	2.084$\pm$4.496\\ \hline
\multirowcell{3}{Duet\\ } &\vone&8.110$\pm$4.252	&	13.000$\pm$4.292	&	14.637$\pm$4.043	\\	  
 &\vtwo& 0.429$\pm$0.896	&	0.890$\pm$1.479	&	1.670$\pm$3.266	\\
 &\vthree& 7.187$\pm$4.284	&	10.440$\pm$4.806	&	12.055$\pm$4.771	\\ \hline
\multirowcell{3}{KNRM\\  } &\vone& 11.543$\pm$6.737	&	18.560$\pm$5.659	&	21.360$\pm$s6.459	 \\ 
 &\vtwo	&6.234$\pm$8.125	&	9.463$\pm$9.408	&	11.211$\pm$10.086\\ 
 &\vthree	&11.114$\pm$6.611	&	17.783$\pm$5.914	&	20.291$\pm$6.500\\ \hline
    \end{tabular}
    \caption{\nrc for MSMarco dataset  }
    \label{table:msmarco_nrc}
\end{table}


\begin{table}[t]
    \centering
    \begin{tabular}{|c|c |c|c |c| }\hline
\textbf{Model} & \textbf{Atk}  & 1 token & 3 tokens & 5 tokens  \\ \hline
\multirowcell{3}{DRMM\\} &\vone& 2.380$\pm$3.252 &	4.009$\pm$4.499& 4.403$\pm$4.753 \\  
&\vtwo& 0.014$\pm$0.118 &0.464$\pm$1.629 & 1.098$\pm$2.943 \\
&\vthree& 1.403$\pm$2.127 & 2.286$\pm$3.160 & 2.455$\pm$3.300 \\ \hline
\multirowcell{3}{Duet\\ } &\vone& 2.175$\pm$2.454 & 3.527$\pm$3.585 &3.773$\pm$3.857	\\	  
 &\vtwo& 	0.040$\pm$0.221 &0.175$\pm$0.506 & 0.366$\pm$0.899	\\
 &\vthree& 	2.005$\pm$2.270 & 3.175$\pm$3.277 & 3.221$\pm$3.280	\\ \hline
\multirowcell{3}{KNRM\\  } &\vone& 1.632$\pm$2.064 &2.580$\pm$2.873 & 2.849$\pm$3.155	 \\ 
 &\vtwo	&0.188$\pm$0.577 & 0.853$\pm$1.647 & 1.160$\pm$2.014\\ 
 &\vthree	&1.575$\pm$1.990 & 2.556$\pm$2.868 & 2.830$\pm$3.084\\ \hline
    \end{tabular}
    \caption{\nrc for WikiQA dataset }
    \label{table:wikiqa_nrc}
\end{table}




==> Adversarial Attack on Rankers/src/intro.tex <==
\section{Introduction}
\label{sec:intro}
% False negative attacks
Deep learning ranking models increasingly represent the state-of-the art in ranking documents with respect to a user query. Different neural architectures \cite{drmm,duet,knrm} are used to model interaction between query and document text to compute relevance. These models rely heavily on the tokens and their embeddings for non-linear transformations for similarity computation. 
% The advantage of using such complex rankers and word embeddings is that they overcome several shortcomings of term-based models such as BM25\cite{bm25} which rely on exact token matches. 
Thus, they capture semantic similarity between query and document tokens circumventing the exact-match limitation of previous models such as BM25~\cite{bm25}. 

The complexity of deep learning models arises from their high dimensional decision boundaries. The hyperplanes are known to be very sensitive to changes in feature values. In computer vision literature \cite{advRank2020} and text based classification tasks \cite{wang2019survey}, researchers have shown that deep learning models can change their predictions with slight variations in inputs. There is a large body of work that investigates adversarial attacks \cite{wang2019survey} on deep networks to quantify their robustness against noise. There is, however, lack of such experiments and evaluation in information retrieval literature. Mitra \emph{et.al.}~\cite{mitra2016dualAdv} demonstrated how word replacement in documents can lead to difference in word representations which leaves room for more investigation of the robustness of deep ranking models to adversarial attacks. 

Usually, adversarial attackers perturb images to reverse a model's decision. Noise addition to images is performed at pixel level such that a human eye cannot distinguish true image from noisy image. In text classification tasks, characters or words \cite{textFool2017,papernot2016crafting} are modified to change the classifier output. 
The objective of the adversary is to reverse model's decision with minimum amount of noise injection. In information retrieval, however, it remains an open problem as to how does one design an adversary for a ranking model. We posit that the objective of an adversary in information retrieval would be to change the position of a document with respect to the query. We follow a similar approach used in text classification tasks \cite{textFool2017,papernot2016crafting} and perturb tokens in documents, replacing them with semantically similar tokens such that the rank of the document changes.

In this work, we demonstrate by means of false negative adversarial attacks that three state-of-the-art retrieval models can change a document's position with slight changes in its text. We evaluate the robustness of these ranking models on publicly available datasets by injecting varied length of noisy text in documents. We propose a black-box adversarial attack model that takes a (query, document) pair as input and generates a noisy document such that its pushed lower in the ranked list. Our system does not need access to the ranker's internal architecture, only its output given the (query, document) tuple as input. 

Our findings suggest that ranking models can be sensitive to even single token perturbations. Table \ref{tab:examples} shows some examples generated by our model of one word perturbations along with changes in document position when scored using state-of-the-art ranking model. 
% We evaluate the robustness of three ranking models on two datasets in this work. 
Overall, we found that simple attackers could perturb very few words and still generate semantically similar text that can fool a model into ranking a relevant document lower than non-relevant documents. 

%\todo{Add numbers and take-away points once we have the results}.


\begin{table}[]
    \centering
    \tiny
    \begin{tabular}{|p{1.5cm}|p{4.2cm}|l|c|}
        \hline
        \textbf{Query} &  \textbf{Relevant Document} & \textbf{Replaced by} & \textbf{$\downarrow$Rank} \\ \hline
        what can be powered by wind 
            & Wind power is the conversion of wind energy into a useful form of energy, such as using wind turbines to make electrical power , windmills for mechanical power, wind pumps for \hone{water} pumping or drainage , or sails to propel ships.
            & \htwo{wind} & 12\\ \hline
        what causes heart disease 
            & The causes of cardiovascular disease are \hone{diverse} but atherosclerosis and/or hypertension are the most common.
            & \htwo{disorder} & 8 \\ \hline
        how many books are included in the protestant Bible? 
            & Christian Bibles range from the sixty-six books of the Protestant \hone{canon} to the eighty-one books of the Ethiopian Orthodox Tewahedo Church canon.
            & \htwo{christian} & 5  \\ \hline
        how many numbers on a credit card 
            & An ISO/IEC 7812 card number is typically 16 digits in \hone{length}, and consists of:
            & \htwo{identification} & 4 \\ \hline
        how many amendments in us  
            & The Constitution has been amended seventeen additional times (for a total of \hone{twenty-seven} amendments).
            & \htwo{allowing} & 4 \\ \hline
        what is a monarch to a monarchy 
            & A monarchy is a form of government in which sovereignty is actually or nominally \hone{embodied} in a single individual (the monarch ).
            & \htwo{throne} & 4  \\ \hline
    \end{tabular}
    \caption{Examples of our one word adversarial perturbation and change in document position when ranked by DRMM.}
    \label{tab:examples}
\end{table}

\section{Related Work}
Adversarial attack on deep neural networks has been extensively explored in vision \cite{onepixel} and text classification \cite{wang2019survey,papernot2016crafting}. Existing work has proposed adversarial attacks with either white-box or black-box access to the model. In this work, our focus is on black-box attacks since access to ranking models is not always available. Existing work is also limited in that the focus is on changing classifier decisions and not document positions in ranked list with respect to a query. In this work we explore utility of (query,doc) pair in adversarial attacks on ranking models. 


\begin{comment}

Main idea: Explain ranker through adversarial attacks
\begin{itemize}
    \item Small perturbation in the document significantly change its rank
    \item Can we say something about the ranker's robustness?
    \item Analyze the perturbed noise (words that need to be changed) to see if they can be used to explain the ranking.
    \item Can we take into account other documents? This way we can be different from attention based approaches that only focus on a single document.
    \item How about query perturbation? 
\end{itemize}
\end{comment}

==> Adversarial Attack on Rankers/src/result_rough.tex <==
\begin{comment}
WIKIQA
DRMM 

v1
	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.204695	0.17638	213	0.138028	0.189114	213	0.307512	0.450059	213
3	0.204695	0.17638	213	0.108920	0.177417	213	0.428404	0.474237	213
5	0.204695	0.17638	213	0.099531	0.173341	213	0.469484	0.476500	213

Non rel crossed

		mean	std	count
length_pert	label			
1	0	4.832222	4.409978	900
1	2.380282	3.252138	213
3	0	7.427778	6.043806	900
1	4.009390	4.499466	213
5	0	7.790000	6.233973	900
1	4.403756	4.753984	213

dpos

		mean	std	count
length_pert	label			
1	0	5.301111	4.649614	900
1	3.549296	3.261216	213
3	0	8.165556	6.320890	900
1	5.352113	4.535287	213
5	0	8.552222	6.519292	900
1	5.751174	4.766141	213


v2

prec
	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.204695	0.17638	213	0.205634	0.176887	213	-0.004695	0.068519	213
3	0.204695	0.17638	213	0.206573	0.196560	213	-0.004695	0.374402	213
5	0.204695	0.17638	213	0.195305	0.196614	213	0.041471	0.423345	213


Non rel crossed

	mean	std	count
length_pert	label			
1	0	0.956667	0.601546	900
1	0.014085	0.118117	213
3	0	1.587778	2.824898	900
1	0.464789	1.629599	213
5	0	2.353333	3.963633	900
1	1.098592	2.943597	213

dpos
	mean	std	count
length_pert	label			
1	0	5.301111	4.649614	900
1	3.549296	3.261216	213
3	0	8.165556	6.320890	900
1	5.352113	4.535287	213
5	0	8.552222	6.519292	900
1	5.751174	4.766141	213

v3
	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.204695	0.17638	213	0.156808	0.186358	213	0.216745	0.400270	213
3	0.204695	0.17638	213	0.138028	0.187108	213	0.304773	0.447740	213
5	0.204695	0.17638	213	0.130516	0.184437	213	0.336463	0.458072	213


Non rel
		mean	std	count
length_pert	label			
1	0	3.310000	2.864479	900
1	1.403756	2.127179	213
3	0	4.957778	4.329889	900
1	2.286385	3.160435	213
5	0	5.188889	4.526020	900
1	2.455399	3.300105	213

dpos
		mean	std	count
length_pert	label			
1	0	3.612222	3.032942	900
1	2.502347	2.142614	213
3	0	5.428889	4.564023	900
1	3.502347	3.248547	213
5	0	5.688889	4.767438	900
1	3.676056	3.376282	213



DUET

v1

	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.207035	0.18021	199	0.150754	0.184738	199	0.244556	0.412273	199
3	0.207035	0.18021	199	0.124623	0.187882	199	0.370184	0.464852	199
5	0.207035	0.18021	199	0.116583	0.184436	199	0.402010	0.468750	199

Non rel crossed
		mean	std	count
length_pert	label			
1	0	4.629103	3.947529	914
1	2.175879	2.454479	199
3	0	6.270241	5.058069	914
1	3.527638	3.585604	199
5	0	6.588621	5.333903	914
1	3.773869	3.857843	199

dpos

	mean	std	count
length_pert	label			
1	0	5.044858	4.103422	914
1	3.412060	2.542777	199
3	0	6.857768	5.243419	914
1	4.879397	3.737001	199
5	0	7.205689	5.519589	914
1	5.160804	4.056952	199

v2
	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.207035	0.18021	199	0.207035	0.183542	199	0.003350	0.074836	199
3	0.207035	0.18021	199	0.215075	0.188492	199	-0.037688	0.237724	199
5	0.207035	0.18021	199	0.208040	0.193677	199	-0.005863	0.322369	199


Non rel

	mean	std	count
length_pert	label			
1	0	0.693654	0.523514	914
1	0.040201	0.221090	199
3	0	1.033917	1.384450	914
1	0.175879	0.506744	199
5	0	1.450766	2.014266	914
1	0.366834	0.899554	199

dpos
	mean	std	count
length_pert	label			
1	0	0.695842	0.563050	914
1	0.683417	0.564323	199
3	0	0.997812	1.585806	914
1	0.824121	0.939708	199
5	0	1.428884	2.229415	914
1	0.984925	1.335140	199


v3

	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.207035	0.18021	199	0.154774	0.184678	199	0.226968	0.402355	199
3	0.207035	0.18021	199	0.128643	0.187309	199	0.350084	0.458733	199
5	0.207035	0.18021	199	0.130653	0.186989	199	0.340034	0.455309	199

Non rel
	mean	std	count
length_pert	label			
1	0	4.399344	3.815177	914
1	2.005025	2.270802	199
3	0	5.871991	4.780393	914
1	3.175879	3.277444	199
5	0	6.128009	4.996825	914
1	3.221106	3.280083	199

dpos
	mean	std	count
length_pert	label			
1	0	4.786652	3.965265	914
1	3.206030	2.314374	199
3	0	6.411379	4.963318	914
1	4.492462	3.434627	199
5	0	6.695842	5.190716	914
1	4.557789	3.499701	199


KNRM 

v1

origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.223585	0.203315	212	0.175472	0.218053	212	0.224057	0.409836	212
3	0.223585	0.203315	212	0.155660	0.215327	212	0.304245	0.445051	212
5	0.223585	0.203315	212	0.147170	0.214722	212	0.341195	0.457160	212

non rel

mean	std	count
length_pert	label			
1	0	2.967814	2.216621	901
1	1.632075	2.064484	212
3	0	4.728080	3.599750	901
1	2.580189	2.873013	212
5	0	5.308546	4.067790	901
1	2.849057	3.155654	212

dpos
	mean	std	count
length_pert	label			
1	0	3.264151	2.379807	901
1	2.849057	2.274076	212
3	0	5.229745	3.801673	901
1	3.929245	3.206878	212
5	0	5.864595	4.276743	901
1	4.202830	3.494260	212

v2
	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.223585	0.203315	212	0.217925	0.206665	212	0.028302	0.166226	212
3	0.223585	0.203315	212	0.203774	0.214155	212	0.089623	0.348528	212
5	0.223585	0.203315	212	0.197170	0.217246	212	0.121069	0.390132	212

non rel changed
	mean	std	count
length_pert	label			
1	0	0.691454	1.062609	901
1	0.188679	0.577841	212
3	0	1.944506	2.147667	901
1	0.853774	1.647153	212
5	0	2.311876	2.488499	901
1	1.160377	2.014811	212

dpos
	mean	std	count
length_pert	label			
1	0	0.724750	1.156498	901
1	0.627358	0.937783	212
3	0	2.067703	2.356285	901
1	1.669811	2.019909	212
5	0	2.480577	2.720888	901
1	2.132075	2.412744	212

v3

origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.223585	0.203315	212	0.176415	0.216850	212	0.218553	0.406220	212
3	0.223585	0.203315	212	0.153774	0.214045	212	0.310535	0.446600	212
5	0.223585	0.203315	212	0.149057	0.214297	212	0.331761	0.453757	212


non rel crossed
	mean	std	count
length_pert	label			
1	0	2.962264	2.216282	901
1	1.575472	1.990252	212
3	0	4.688124	3.567658	901
1	2.556604	2.868625	212
5	0	5.215316	4.041208	901
1	2.830189	3.084810	212

dpos
	mean	std	count
length_pert	label			
1	0	3.256382	2.385087	901
1	2.787736	2.185094	212
3	0	5.184240	3.776156	901
1	3.905660	3.202571	212
5	0	5.755827	4.256274	901
1	4.193396	3.456617	212

MSMARCO

DRMM 

v1

	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.801714	0.194333	700	0.773143	0.218380	700	0.049048	0.144699	700
3	0.801714	0.194333	700	0.723429	0.220468	700	0.113690	0.175213	700
5	0.801714	0.194333	700	0.688000	0.219569	700	0.160238	0.177973	700


mean	std	count
length_pert	label			
1	0	4.681928	4.104320	415
1	0.944286	2.776054	700
3	0	11.221687	7.241121	415
1	3.867143	6.334347	700
5	0	14.561446	7.755345	415
1	6.814286	7.857990	700

dpos
		mean	std	count
length_pert	label			
1	0	5.253012	4.548832	415
1	2.722857	2.922028	700
3	0	12.337349	7.937676	415
1	6.307143	6.257123	700
5	0	15.855422	8.440660	415
1	9.467143	7.685358	700

v2

	mean	std	count
length_pert			
1	0.000881	0.059361	700
3	0.015429	0.110500	700
5	0.023024	0.127322	700

	origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert 						
1	0.801714	0.194333	700	0.801143	0.195219	700
3	0.801714	0.194333	700	0.794286	0.205424	700
5	0.801714	0.194333	700	0.790571	0.206814	700

	mean	std	count
length_pert	label			
1	0	0.865060	1.002947	415
1	0.037143	0.622692	700
3	0	2.330120	4.216305	415
1	0.304286	1.752247	700
5	0	2.944578	4.779112	415
1	0.647143	3.128585	700

	mean	std	count
length_pert	label			
1	0	0.874699	1.203341	415
1	0.821429	0.979532	700
3	0	2.522892	4.745079	415
1	1.272857	2.049071	700
5	0	3.265060	5.405947	415
1	1.882857	3.460464	700
v3

	mean	std	count
length_pert			
1	0.029452	0.119264	700
3	0.061500*	0.156141	700
5	0.076000*	0.162744	700


origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.801714	0.194333	700	0.785143	0.209111	700
3	0.801714	0.194333	700	0.763429	0.216698	700
5	0.801714	0.194333	700	0.752000	0.217369	700

num non rel

mean	std	count
length_pert	label			
1	0	2.956627	2.628908	415
1	0.404286	1.730227	700
3	0	5.821687	4.740820	415
1	1.280000	3.388342	700
5	0	7.915663	5.973381	415
1	2.084286	4.495750	700

dpos

		mean	std	count
length_pert	label			
1	0	3.214458	2.692768	415
1	1.838571	1.881602	700
3	0	6.303614	4.802813	415
1	3.087143	3.451624	700
5	0	8.546988	6.020664	415
1	4.055714	4.556249	700

DUET

v1

	mean	std	count
length_pert			
1	0.598901	0.400600	91
3	0.684982	0.353510	91
5	0.703297	0.335918	91

	origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.318681	0.151959	91	0.160440	0.171839	91
3	0.318681	0.151959	91	0.138462	0.165173	91
5	0.318681	0.151959	91	0.131868	0.155549	91


	mean	std	count
length_pert	label			
1	0	8.695312	3.845366	1024
1	8.109890	4.251668	91
3	0	13.027344	4.089568	1024
1	13.000000	4.292112	91
5	0	14.680664	4.183776	1024
1	14.637363	4.042872	91


dpos
	mean	std	count
length_pert	label			
1	0	9.301758	4.154842	1024
1	9.890110	4.539825	91
3	0	14.058594	4.427595	1024
1	15.307692	4.401243	91
5	0	15.896484	4.525698	1024
1	17.142857	4.334798	91


v2

	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.318681	0.151959	91	0.309890	0.164016	91	0.023810	0.300793	91
3	0.318681	0.151959	91	0.305495	0.174714	91	0.029304	0.465205	91
5	0.318681	0.151959	91	0.290110	0.198357	91	0.122711	0.469328	91

		mean	std	count
length_pert	label			
1	0	0.875977	1.087227	1024
1	0.428571	0.896200	91
3	0	1.486328	2.035801	1024
1	0.890110	1.479118	91
5	0	1.783203	2.376957	1024
1	1.670330	3.266173	91

dpos

		mean	std	count
length_pert	label			
1	0	0.770508	1.288747	1024
1	1.010989	1.441408	91
3	0	1.324219	2.372941	1024
1	1.384615	2.184639	91
5	0	1.599609	2.789773	1024
1	2.230769	3.921669	91

v3
	mean	std	count
length_pert			
1	0.560440	0.404844	91
3	0.615385	0.392595	91
5	0.659341	0.369277	91

	origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.318681	0.151959	91	0.167033	0.166703	91
3	0.318681	0.151959	91	0.156044	0.170756	91
5	0.318681	0.151959	91	0.145055	0.168828	91

	mean	std	count
length_pert	label			
1	0	8.542969	3.884464	1024
1	7.186813	4.284110	91
3	0	12.485352	4.333121	1024
1	10.439560	4.805573	91
5	0	14.015625	4.379566	1024
1	12.054945	4.771123	91

dpos

mean	std	count
length_pert	label			
1	0	9.132812	4.203050	1024
1	8.857143	4.540121	91
3	0	13.460938	4.675432	1024
1	12.505495	5.192674	91
5	0	15.154297	4.757216	1024
1	14.230769	5.064203	91

KNRM

v1

	mean	std	count
length_pert			
1	0.532381	0.374898	175
3	0.594286	0.339971	175
5	0.594286	0.339971	175

	origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.373714	0.175497	175	0.213714	0.193680	175
3	0.373714	0.175497	175	0.194286	0.188678	175
5	0.373714	0.175497	175	0.194286	0.188678	175

		mean	std	count
length_pert	label			
1	0	13.988298	6.602906	940
1	11.542857	6.737026	175
3	0	22.238298	7.278619	940
1	18.560000	5.659455	175
5	0	25.685106	7.240490	940
1	21.360000	6.458675	175

dpos
		mean	std	count
length_pert	label			
1	0	15.807447	7.375675	940
1	14.251429	7.425855	175
3	0	25.131915	8.018990	940
1	22.160000	5.942019	175
5	0	29.001064	7.880294	940
1	25.137143	6.640484	175

v2
	mean	std	count
length_pert			
1	0.300000	0.420386	175
3	0.387143	0.431907	175
5	0.417143	0.426371	175

	origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.373714	0.175497	175	0.291429	0.215187	175
3	0.373714	0.175497	175	0.264000	0.215535	175
5	0.373714	0.175497	175	0.252571	0.210040	175

	mean	std	count
length_pert	label			
1	0	7.914894	8.345903	940
1	6.234286	8.125239	175
3	0	14.189362	10.517002	940
1	9.462857	9.407599	175
5	0	16.492553	10.535045	940
1	11.211429	10.085604	175

dpos
		mean	std	count
length_pert	label			
1	0	8.855319	9.456944	940
1	7.988571	9.148198	175
3	0	15.986170	11.867965	940
1	11.622857	10.599043	175
5	0	18.610638	11.838705	940
1	13.617143	11.333337	175

v3

	mean	std	count
length_pert			
1	0.525714	0.380695	175
3	0.594286	0.339971	175
5	0.594286	0.339971	175


origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.373714	0.175497	175	0.217143	0.197522	175
3	0.373714	0.175497	175	0.194286	0.188678	175
5	0.373714	0.175497	175	0.194286	0.188678	175

	mean	std	count
length_pert	label			
1	0	14.071277	6.743926	940
1	11.114286	6.610560	175
3	0	22.126596	7.181945	940
1	17.782857	5.914014	175
5	0	25.192553	7.269947	940
1	20.291429	6.500282	175


dpos

		mean	std	count
length_pert	label			
1	0	15.873404	7.558641	940
1	13.788571	7.275837	175
3	0	25.031915	7.883540	940
1	21.234286	6.393870	175
5	0	28.454255	7.942889	940
1	23.942857	6.926307	175



DRMM
MSMARco

mean dist -- label =1 nqchange > 0

v1
mean	std	count
length_pert			
1	0.841288	0.147450	540
3	0.966052	0.064321	634
5	1.024848	0.041315	322




##### RANK DROP SUCCESS ####
WIKIQA
DRMM
PLEN    1       3       5
V1@1    100     100     100
V1@3    49.7    70.4    73.7
V1@5    25.8    45      48.8

PLEN    1       3       5
V2@1    92.5    62.4    70.4
V2@3    0       9.9     19.7
V2@5    0       2.3     8.9

PLEN    1       3       5
V3@1    100     100     100
V3@3    33.3    49.8    51.6
V3@5    15      24.9    26.8

V0@1
3    0.888393
5    1.236607

V0@3
3    0.566964
5    0.620536

v0@5
3    0.357143
5    0.383929

###DUET###

V0@1
3    1.000000
5    1.386935

V0@3
3    0.668342
5    0.708543

v0@5
3    0.422111
5    0.472362


V1@1
1    1.0
3    1.0
5    1.0

V1@3
1    0.512563
3    0.668342
5    0.668342

V1@5
1    0.266332
3    0.422111
5    0.467337

V2@1
1    0.648241
3    0.678392
5    0.683417

V2@3
1    0.005025
3    0.050251
5    0.090452

V2@5
3    0.005025
5    0.035176

V3@1
1    1.0
3    1.0
5    1.0

V3@3
1    0.497487
3    0.638191
5    0.643216

V3@5
1    0.251256
3    0.396985
5    0.402010


##KNRM##
V0@1

V0@3

v0@5


V1@1
1    1.0
3    1.0
5    1.0

V1@3
1    0.438679
3    0.599057
5    0.608491

V1@5
1    0.127358
3    0.297170
5    0.316038

V2@1
1    0.405660
3    0.773585
5    0.844340

V2@3
1    0.042453
3    0.231132
5    0.273585

V2@5
1    0.009434
3    0.051887
5    0.122642

V3@1
1    1.0
3    1.0
5    1.0

V3@3
1    0.424528
3    0.589623
5    0.617925

V3@5
1    0.132075
3    0.297170
5    0.316038

MSMARCO
DRMM
PLEN    1       3       5
V1@1    100     100     100
V1@3    32.9    75.9    90.1
V1@5    11.4    40.6    65.6

PLEN    1       3       5
V2@1    73.3    76.1    84.1
V2@3    1.7     8.3     15
V2@5    0.3     3.4     4.4

PLEN    1       3       5
V3@1    100     100     100
V3@3    15.7    38.9    49.2
V3@5    4       14.6    24.2

V0@1

V0@3

v0@5

DUET
V0@1

V0@3

v0@5


V1@1
1    1.0
3    1.0
5    1.0

V1@3
1    0.934066
3    1.000000
5    1.000000

V1@5
1    0.868132
3    0.967033
5    1.000000

V2@1
1    0.571429
3    0.571429
5    0.659341

V2@3
1    0.153846
3    0.285714
5    0.340659

V2@5
1    0.032967
3    0.098901
5    0.186813

V3@1
1    1.0
3    1.0
5    1.0

V3@3
1    0.934066
3    0.945055
5    0.978022

V3@5
1    0.813187
3    0.879121
5    0.934066


KNRM
V0@1

V0@3

v0@5


V1@1
length_pert
1    1.0
3    1.0
5    1.0

V1@3
1    0.971429
3    1.000000
5    1.000000

V1@5
1    0.897143
3    1.000000
5    1.000000

V2@1
1    0.891429
3    0.891429
5    0.942857

V2@3
1    0.520000
3    0.662857
5    0.742857

V2@5
1    0.451429
3    0.582857
5    0.668571

V3@1
1    1.0
3    1.0
5    1.0

V3@3
1    0.977143
3    1.000000
5    1.000000

V3@5
1    0.891429
3    1.000000
5    1.000000



\begin{comment}
% \small{$^+=pval<0.10$ and $^*=pval<0.05$ with 2 tailed ttest}}
\begin{comment}
\begin{table}[]
    \centering
    \begin{tabular}{ |c| c| c| }
 DRMM & Duet & KNRM \\ 
 cell4 & cell5 & cell6 \\  
 cell7 & cell8 & cell9    
    \end{tabular}
    \caption{Caption}
    \label{table:ranker_config}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c |c|c|c | }\hline
\textbf{Model} & \textbf{Fit}  & \multicolumn{3}{|c|}{WikiQA}   \\ \hline
\multirow{3}{*}{DRMM}  &v1& 0.977$\pm$0.003 & 0.927$\pm$0.005 & 0.878 $\pm$0.006  \\  
 &v2& 0.986$\pm$0.007 & 0.944$\pm$0.014 & 0.879$\pm$0.007\\
 &v3&0.977$\pm$0.003  & 0.953$\pm$0.004& 0.879$\pm$0.007\\ \hline
\multirow{3}{*}{KNRM} &v1& 0.978$\pm$0.004 & 0.930$\pm$0.005  & 	0.881$\pm$0.006  \\ 
 &v2& 0.989$\pm$0.007 & 0.948$\pm$0.009  & 0.911$\pm$0.006  \\ 
 &v3& 0.978$\pm$0.004 & 0.929$\pm$0.005  & 0.880$\pm$0.006 \\ \hline
 \multirow{3}{*}{Duet} &v1& 0.974$\pm$0.002 & 0.925$\pm$0.004  & 0.877$\pm$0.005  \\ 
 &v2& 0.986$\pm$0.007 & 0.947$\pm$0.010  & 0.913$\pm$0.005   \\ 
 &v3& 0.974$\pm$0.002 & 0.926$\pm$0.004  & 0.877$\pm$0.006 \\ \hline
    \end{tabular}
    \caption{Emb sim b/w perturbed \& original WikiQA ans}
    \label{table:wikiqa_cosine}
\end{table}

\end{comment}


==> Adversarial Attack on Rankers/src/results.tex <==
\section{Results and Discussion}
We focus on three research questions to investigate the impact of adversarial attacks on ranking models.\newline
\textbf{RQ1:} \emph{What is the attacker's success in changing a document's position without significantly changing the document?}
To answer this question, we measure an attacker's success (\sk) 
when we restrict the number of perturbed words to \textit{one} in each document.  The results for $k=1$ and $k=5$ are given in Table~\ref{table:success}. Notice that \vzero can change the rank of almost half of the relevant documents but not beyond five positions.
Both \vone and \vthree can change the rank of all the relevant documents by just changing \emph{one term} in the document. 
In case of MSMarco, they can lower the rank of >81\% relevant documents by more than four positions except for DRMM ranker.
Overall, we found that \vone has the highest success rate among all the attackers as it has greater flexibility to change the terms. 

We report mean and variance of \nrc on the test sets in Table~\ref{table:msmarco_nrc} and~\ref{table:wikiqa_nrc} for MSMarco and WikiQA datasets respectively.
Increasing the number of perturbed words increases \nrc across all the attackers. On MSMarco dataset, KNRM is the most vulnerable ranker across all the attackers. On average \vone can push a relevant document beyond 11 non-relevant documents by changing only one token when evaluated against KNRM ranker. On the other hand, the performance of attackers across all the models is similar on the WikiQA dataset.
Overall, all the attackers perform better on MSMarco dataset compared to WikiQA. We argue that the larger length of passages in MSMarco provides more room for perturbations as opposed to the shorter length of answers in WikiQA. \newline
\textbf{RQ2:} \emph{What is the similarity between perturbed and original text when we restrict the number of perturbed words to $p_l=\{1,3,5\}$ in each document?} 
%We explore cosine similarity between perturbed and original text.
Adversarial perturbations may cause the meaning of document text to change. Thus, it is important to control this change such that perturbed words are semantically similar to original text. We measure the semantic similarity between embeddings of original text and perturbed text using cosine distance as done in previous work \cite{wang2019survey}. Figure \ref{fig:dc} shows similarity b/w perturbed and original text when 1, 3 or 5 tokens are changed in MSMarco passage text for three different models. 
% Token embeddings will vary across models as embedding weights were tuned, along with other parameters, for both datasets separately. 
We only focus on similarity for \vone and \vthree attackers due to space limitations. 

Overall, the cosine similarity between perturbed and original text across attackers is relatively high ($\sim$0.97), even though the document may be pushed below $\sim$20 non-relevant documents with only \emph{single} token perturbations. As expected, perturbing more tokens leads to lower similarity. Cosine similarity drops to $\sim$0.90 across models for 5 word perturbations. Both \vone and \vthree attackers can push documents to relatively lower positions with 1-3 token perturbations, however, we found that \vone tends to perturb query tokens in passages to change ranker output. We found that \vone changed query tokens in 65\% (DRMM), 11\% (Duet) and 2\% (KNRM) documents in MSMarco and  50\%, 17\% and 3\% documents in WikiQA respectively. However, \vthree achieves similar performance in terms of similarity and rank change \emph{without} changing any query tokens. \newline
%We observe similar results on WikiQA but omit them due to lack of space.
\captionsetup[figure*]{font=tiny}
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{fig/msmarco_drmm_v1.png}
        %{images/uniform_01_FT924-8062.png}
        \caption{DRMM (\vone)}
        \label{fig:drmm_v1}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{fig/msmarco_duet_v1.png}
        \caption{DUET (\vone)}
        \label{fig:duet_v1}
    \end{subfigure}
      \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{fig/msmarco_knrm_v1.png}
        \caption{KNRM (\vone)}
        \label{fig:knrm_v1}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{fig/msmarco_drmm_v3.png}
        %{images/uniform_01_FT924-8062.png}
        \caption{DRMM (\vthree)}
        \label{fig:drmm_v3}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{fig/msmarco_duet_v3.png}
        \caption{DUET (\vthree)}
        \label{fig:duet_v3}
    \end{subfigure}
      \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{fig/msmarco_knrm_v3.png}
        \caption{KNRM (\vthree)}
        \label{fig:knrm_v3}
    \end{subfigure}
\caption{\small{\nrc vs. cosine sim on MSMarco where {\color{CornflowerBlue} blue=1 word}, {\color{Peach} orange=3 words} and {\color{ForestGreen} green=5 words} perturbations respectively.}}
    \label{fig:dc}
\end{figure}
\begin{table}[t]
    \centering
    \begin{tabular}{|c|c |c|c |c|c | }\hline
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Atk}}  & \multicolumn{2}{|c|}{WikiQA} &  \multicolumn{2}{|c|}{MSMarco} \\ \cline{3-6}
 &   & 1 token & 3 tokens  & 1 token & 3 tokens   \\ \hline
\multirow{3}{*}{DRMM}  &\vone &0.31$\pm$0.45	&	0.43$\pm$0.47&	0.05$\pm$0.14	&	0.11$\pm$0.17 \\  
 &\vtwo&0.005$\pm$0.06	&	0.005$\pm$0.37&	0.001$\pm$0.05	&	0.01$\pm$0.11\\
 &\vthree&0.216$\pm$0.40	&	0.30$\pm$0.44 &	0.02$\pm$0.11	&	0.06$\pm$0.15\\ \hline
\multirow{3}{*}{Duet} &\vone& 0.24$\pm$0.41	&	0.37$\pm$0.46 &	0.59$\pm$0.40	&	0.68$\pm$0.35\\
 &\vtwo& 0.003$\pm$0.07	&	-0.04$\pm$0.23 &	0.02$\pm$0.30	&	0.03$\pm$0.46 \\ 
 &\vthree& 0.226$\pm$0.40	&	0.35$\pm$0.45&	0.56$\pm$0.40	&	0.61$\pm$0.39\\ \hline
 \multirow{3}{*}{KNRM} &\vone&0.22$\pm$0.41	&	0.30$\pm$0.44&	0.53$\pm$0.37	&	0.59$\pm$0.34\\ 
 &\vtwo&0.03$\pm$0.16	&0.09$\pm$0.34&0.30$\pm$0.42&0.38$\pm$0.43 \\ 
 &\vthree&0.218$\pm$0.40	&	0.31$\pm$0.44 &	0.52$\pm$0.38	&	0.59$\pm$0.34\\ \hline
    \end{tabular}
    \caption{\% drop in $P@5$ due to perturbed text}
    \label{table:prec_drop}
\end{table}
\textbf{RQ3:} \emph{What is the ranker performance after adversarial attacks?} We evaluate model robustness against an adversarial attacker with P@5. 
% We compute perturbed $P@5$ by replacing the original document's $d_i$ ranker score $s_i$ with the new score $\hat{s_i}$ given by the ranker with the perturbed document $\hat{d_i}$ from the attacker as input.
We compute perturbed $P@5$ by replacing the original document's ($d_i$) ranker score $s_i$ with the new score $s'_i$ given by the ranker on the perturbed input $d'_i$.
\footnote{Note that ranker output for all other documents in the list  $d_{j\neq i}$ remains the same.} So, for every document the attacker perturbs, its new score replaces the old ranker score and $P@5$ is recomputed. We report the \% drop in $P@5$ for both datasets in Table \ref{table:prec_drop}. 
%\small{$^+=pval<0.10$ and $^*=pval<0.05$ with 2 tailed ttest}}
We find that \vone and \vthree attackers are able to reduce $P@5$ significantly, in some cases as much as $\sim$20\% in WikiQA and $\sim$50\% in MSMarco by changing one token in the text. Although, \vthree's drop in $P@5$ is lower than that of \vone's across all datasets since it is penalized for changing query terms. 

We also found \%drop in $P@5$ to be a function of ranker performance. Models with higher precision were harder to beat by the attacker, i.e., were more robust to token changes in document text. For example, in WikiQA original $P@5$ (mean,std) for DRMM, Duet and KNRM was 0.204$\pm$0.17, 0.207$\pm$0.18 and 0.22$\pm$0.20 respectively. It is interesting to note that all attackers are able to reduce DRMM $P@5$ by single token perturbations by highest margin. However, in MSMarco, DRMM $P@5$ is the highest amongst all other models, thus hardest to fool by all attackers. We observe very little drop in precision for \vtwo attacker across models in both datasets which indicates that very strict attackers may not be able to find suitable candidates to perturb documents. One interesting finding was that in some cases the attacker replaced document text with \emph{query tokens} to lower document score as shown in Table \ref{tab:examples}. 




%\textbf{RQ3:} Finally, we explore whether relevant documents are more immune to adversarial attacks compared to non-relevant documents. The underlying hypothesis is that small changes in relevant documents should not change their position in the list drastically. 






==> src/result_rough.tex <==
\begin{comment}
WIKIQA
DRMM 

v1
	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.204695	0.17638	213	0.138028	0.189114	213	0.307512	0.450059	213
3	0.204695	0.17638	213	0.108920	0.177417	213	0.428404	0.474237	213
5	0.204695	0.17638	213	0.099531	0.173341	213	0.469484	0.476500	213

Non rel crossed

		mean	std	count
length_pert	label			
1	0	4.832222	4.409978	900
1	2.380282	3.252138	213
3	0	7.427778	6.043806	900
1	4.009390	4.499466	213
5	0	7.790000	6.233973	900
1	4.403756	4.753984	213

dpos

		mean	std	count
length_pert	label			
1	0	5.301111	4.649614	900
1	3.549296	3.261216	213
3	0	8.165556	6.320890	900
1	5.352113	4.535287	213
5	0	8.552222	6.519292	900
1	5.751174	4.766141	213


v2

prec
	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.204695	0.17638	213	0.205634	0.176887	213	-0.004695	0.068519	213
3	0.204695	0.17638	213	0.206573	0.196560	213	-0.004695	0.374402	213
5	0.204695	0.17638	213	0.195305	0.196614	213	0.041471	0.423345	213


Non rel crossed

	mean	std	count
length_pert	label			
1	0	0.956667	0.601546	900
1	0.014085	0.118117	213
3	0	1.587778	2.824898	900
1	0.464789	1.629599	213
5	0	2.353333	3.963633	900
1	1.098592	2.943597	213

dpos
	mean	std	count
length_pert	label			
1	0	5.301111	4.649614	900
1	3.549296	3.261216	213
3	0	8.165556	6.320890	900
1	5.352113	4.535287	213
5	0	8.552222	6.519292	900
1	5.751174	4.766141	213

v3
	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.204695	0.17638	213	0.156808	0.186358	213	0.216745	0.400270	213
3	0.204695	0.17638	213	0.138028	0.187108	213	0.304773	0.447740	213
5	0.204695	0.17638	213	0.130516	0.184437	213	0.336463	0.458072	213


Non rel
		mean	std	count
length_pert	label			
1	0	3.310000	2.864479	900
1	1.403756	2.127179	213
3	0	4.957778	4.329889	900
1	2.286385	3.160435	213
5	0	5.188889	4.526020	900
1	2.455399	3.300105	213

dpos
		mean	std	count
length_pert	label			
1	0	3.612222	3.032942	900
1	2.502347	2.142614	213
3	0	5.428889	4.564023	900
1	3.502347	3.248547	213
5	0	5.688889	4.767438	900
1	3.676056	3.376282	213



DUET

v1

	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.207035	0.18021	199	0.150754	0.184738	199	0.244556	0.412273	199
3	0.207035	0.18021	199	0.124623	0.187882	199	0.370184	0.464852	199
5	0.207035	0.18021	199	0.116583	0.184436	199	0.402010	0.468750	199

Non rel crossed
		mean	std	count
length_pert	label			
1	0	4.629103	3.947529	914
1	2.175879	2.454479	199
3	0	6.270241	5.058069	914
1	3.527638	3.585604	199
5	0	6.588621	5.333903	914
1	3.773869	3.857843	199

dpos

	mean	std	count
length_pert	label			
1	0	5.044858	4.103422	914
1	3.412060	2.542777	199
3	0	6.857768	5.243419	914
1	4.879397	3.737001	199
5	0	7.205689	5.519589	914
1	5.160804	4.056952	199

v2
	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.207035	0.18021	199	0.207035	0.183542	199	0.003350	0.074836	199
3	0.207035	0.18021	199	0.215075	0.188492	199	-0.037688	0.237724	199
5	0.207035	0.18021	199	0.208040	0.193677	199	-0.005863	0.322369	199


Non rel

	mean	std	count
length_pert	label			
1	0	0.693654	0.523514	914
1	0.040201	0.221090	199
3	0	1.033917	1.384450	914
1	0.175879	0.506744	199
5	0	1.450766	2.014266	914
1	0.366834	0.899554	199

dpos
	mean	std	count
length_pert	label			
1	0	0.695842	0.563050	914
1	0.683417	0.564323	199
3	0	0.997812	1.585806	914
1	0.824121	0.939708	199
5	0	1.428884	2.229415	914
1	0.984925	1.335140	199


v3

	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.207035	0.18021	199	0.154774	0.184678	199	0.226968	0.402355	199
3	0.207035	0.18021	199	0.128643	0.187309	199	0.350084	0.458733	199
5	0.207035	0.18021	199	0.130653	0.186989	199	0.340034	0.455309	199

Non rel
	mean	std	count
length_pert	label			
1	0	4.399344	3.815177	914
1	2.005025	2.270802	199
3	0	5.871991	4.780393	914
1	3.175879	3.277444	199
5	0	6.128009	4.996825	914
1	3.221106	3.280083	199

dpos
	mean	std	count
length_pert	label			
1	0	4.786652	3.965265	914
1	3.206030	2.314374	199
3	0	6.411379	4.963318	914
1	4.492462	3.434627	199
5	0	6.695842	5.190716	914
1	4.557789	3.499701	199


KNRM 

v1

origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.223585	0.203315	212	0.175472	0.218053	212	0.224057	0.409836	212
3	0.223585	0.203315	212	0.155660	0.215327	212	0.304245	0.445051	212
5	0.223585	0.203315	212	0.147170	0.214722	212	0.341195	0.457160	212

non rel

mean	std	count
length_pert	label			
1	0	2.967814	2.216621	901
1	1.632075	2.064484	212
3	0	4.728080	3.599750	901
1	2.580189	2.873013	212
5	0	5.308546	4.067790	901
1	2.849057	3.155654	212

dpos
	mean	std	count
length_pert	label			
1	0	3.264151	2.379807	901
1	2.849057	2.274076	212
3	0	5.229745	3.801673	901
1	3.929245	3.206878	212
5	0	5.864595	4.276743	901
1	4.202830	3.494260	212

v2
	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.223585	0.203315	212	0.217925	0.206665	212	0.028302	0.166226	212
3	0.223585	0.203315	212	0.203774	0.214155	212	0.089623	0.348528	212
5	0.223585	0.203315	212	0.197170	0.217246	212	0.121069	0.390132	212

non rel changed
	mean	std	count
length_pert	label			
1	0	0.691454	1.062609	901
1	0.188679	0.577841	212
3	0	1.944506	2.147667	901
1	0.853774	1.647153	212
5	0	2.311876	2.488499	901
1	1.160377	2.014811	212

dpos
	mean	std	count
length_pert	label			
1	0	0.724750	1.156498	901
1	0.627358	0.937783	212
3	0	2.067703	2.356285	901
1	1.669811	2.019909	212
5	0	2.480577	2.720888	901
1	2.132075	2.412744	212

v3

origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.223585	0.203315	212	0.176415	0.216850	212	0.218553	0.406220	212
3	0.223585	0.203315	212	0.153774	0.214045	212	0.310535	0.446600	212
5	0.223585	0.203315	212	0.149057	0.214297	212	0.331761	0.453757	212


non rel crossed
	mean	std	count
length_pert	label			
1	0	2.962264	2.216282	901
1	1.575472	1.990252	212
3	0	4.688124	3.567658	901
1	2.556604	2.868625	212
5	0	5.215316	4.041208	901
1	2.830189	3.084810	212

dpos
	mean	std	count
length_pert	label			
1	0	3.256382	2.385087	901
1	2.787736	2.185094	212
3	0	5.184240	3.776156	901
1	3.905660	3.202571	212
5	0	5.755827	4.256274	901
1	4.193396	3.456617	212

MSMARCO

DRMM 

v1

	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.801714	0.194333	700	0.773143	0.218380	700	0.049048	0.144699	700
3	0.801714	0.194333	700	0.723429	0.220468	700	0.113690	0.175213	700
5	0.801714	0.194333	700	0.688000	0.219569	700	0.160238	0.177973	700


mean	std	count
length_pert	label			
1	0	4.681928	4.104320	415
1	0.944286	2.776054	700
3	0	11.221687	7.241121	415
1	3.867143	6.334347	700
5	0	14.561446	7.755345	415
1	6.814286	7.857990	700

dpos
		mean	std	count
length_pert	label			
1	0	5.253012	4.548832	415
1	2.722857	2.922028	700
3	0	12.337349	7.937676	415
1	6.307143	6.257123	700
5	0	15.855422	8.440660	415
1	9.467143	7.685358	700

v2

	mean	std	count
length_pert			
1	0.000881	0.059361	700
3	0.015429	0.110500	700
5	0.023024	0.127322	700

	origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert 						
1	0.801714	0.194333	700	0.801143	0.195219	700
3	0.801714	0.194333	700	0.794286	0.205424	700
5	0.801714	0.194333	700	0.790571	0.206814	700

	mean	std	count
length_pert	label			
1	0	0.865060	1.002947	415
1	0.037143	0.622692	700
3	0	2.330120	4.216305	415
1	0.304286	1.752247	700
5	0	2.944578	4.779112	415
1	0.647143	3.128585	700

	mean	std	count
length_pert	label			
1	0	0.874699	1.203341	415
1	0.821429	0.979532	700
3	0	2.522892	4.745079	415
1	1.272857	2.049071	700
5	0	3.265060	5.405947	415
1	1.882857	3.460464	700
v3

	mean	std	count
length_pert			
1	0.029452	0.119264	700
3	0.061500*	0.156141	700
5	0.076000*	0.162744	700


origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.801714	0.194333	700	0.785143	0.209111	700
3	0.801714	0.194333	700	0.763429	0.216698	700
5	0.801714	0.194333	700	0.752000	0.217369	700

num non rel

mean	std	count
length_pert	label			
1	0	2.956627	2.628908	415
1	0.404286	1.730227	700
3	0	5.821687	4.740820	415
1	1.280000	3.388342	700
5	0	7.915663	5.973381	415
1	2.084286	4.495750	700

dpos

		mean	std	count
length_pert	label			
1	0	3.214458	2.692768	415
1	1.838571	1.881602	700
3	0	6.303614	4.802813	415
1	3.087143	3.451624	700
5	0	8.546988	6.020664	415
1	4.055714	4.556249	700

DUET

v1

	mean	std	count
length_pert			
1	0.598901	0.400600	91
3	0.684982	0.353510	91
5	0.703297	0.335918	91

	origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.318681	0.151959	91	0.160440	0.171839	91
3	0.318681	0.151959	91	0.138462	0.165173	91
5	0.318681	0.151959	91	0.131868	0.155549	91


	mean	std	count
length_pert	label			
1	0	8.695312	3.845366	1024
1	8.109890	4.251668	91
3	0	13.027344	4.089568	1024
1	13.000000	4.292112	91
5	0	14.680664	4.183776	1024
1	14.637363	4.042872	91


dpos
	mean	std	count
length_pert	label			
1	0	9.301758	4.154842	1024
1	9.890110	4.539825	91
3	0	14.058594	4.427595	1024
1	15.307692	4.401243	91
5	0	15.896484	4.525698	1024
1	17.142857	4.334798	91


v2

	origprec@5	pertprec@5	perc_prec
mean	std	count	mean	std	count	mean	std	count
length_pert									
1	0.318681	0.151959	91	0.309890	0.164016	91	0.023810	0.300793	91
3	0.318681	0.151959	91	0.305495	0.174714	91	0.029304	0.465205	91
5	0.318681	0.151959	91	0.290110	0.198357	91	0.122711	0.469328	91

		mean	std	count
length_pert	label			
1	0	0.875977	1.087227	1024
1	0.428571	0.896200	91
3	0	1.486328	2.035801	1024
1	0.890110	1.479118	91
5	0	1.783203	2.376957	1024
1	1.670330	3.266173	91

dpos

		mean	std	count
length_pert	label			
1	0	0.770508	1.288747	1024
1	1.010989	1.441408	91
3	0	1.324219	2.372941	1024
1	1.384615	2.184639	91
5	0	1.599609	2.789773	1024
1	2.230769	3.921669	91

v3
	mean	std	count
length_pert			
1	0.560440	0.404844	91
3	0.615385	0.392595	91
5	0.659341	0.369277	91

	origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.318681	0.151959	91	0.167033	0.166703	91
3	0.318681	0.151959	91	0.156044	0.170756	91
5	0.318681	0.151959	91	0.145055	0.168828	91

	mean	std	count
length_pert	label			
1	0	8.542969	3.884464	1024
1	7.186813	4.284110	91
3	0	12.485352	4.333121	1024
1	10.439560	4.805573	91
5	0	14.015625	4.379566	1024
1	12.054945	4.771123	91

dpos

mean	std	count
length_pert	label			
1	0	9.132812	4.203050	1024
1	8.857143	4.540121	91
3	0	13.460938	4.675432	1024
1	12.505495	5.192674	91
5	0	15.154297	4.757216	1024
1	14.230769	5.064203	91

KNRM

v1

	mean	std	count
length_pert			
1	0.532381	0.374898	175
3	0.594286	0.339971	175
5	0.594286	0.339971	175

	origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.373714	0.175497	175	0.213714	0.193680	175
3	0.373714	0.175497	175	0.194286	0.188678	175
5	0.373714	0.175497	175	0.194286	0.188678	175

		mean	std	count
length_pert	label			
1	0	13.988298	6.602906	940
1	11.542857	6.737026	175
3	0	22.238298	7.278619	940
1	18.560000	5.659455	175
5	0	25.685106	7.240490	940
1	21.360000	6.458675	175

dpos
		mean	std	count
length_pert	label			
1	0	15.807447	7.375675	940
1	14.251429	7.425855	175
3	0	25.131915	8.018990	940
1	22.160000	5.942019	175
5	0	29.001064	7.880294	940
1	25.137143	6.640484	175

v2
	mean	std	count
length_pert			
1	0.300000	0.420386	175
3	0.387143	0.431907	175
5	0.417143	0.426371	175

	origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.373714	0.175497	175	0.291429	0.215187	175
3	0.373714	0.175497	175	0.264000	0.215535	175
5	0.373714	0.175497	175	0.252571	0.210040	175

	mean	std	count
length_pert	label			
1	0	7.914894	8.345903	940
1	6.234286	8.125239	175
3	0	14.189362	10.517002	940
1	9.462857	9.407599	175
5	0	16.492553	10.535045	940
1	11.211429	10.085604	175

dpos
		mean	std	count
length_pert	label			
1	0	8.855319	9.456944	940
1	7.988571	9.148198	175
3	0	15.986170	11.867965	940
1	11.622857	10.599043	175
5	0	18.610638	11.838705	940
1	13.617143	11.333337	175

v3

	mean	std	count
length_pert			
1	0.525714	0.380695	175
3	0.594286	0.339971	175
5	0.594286	0.339971	175


origprec@5	pertprec@5
mean	std	count	mean	std	count
length_pert						
1	0.373714	0.175497	175	0.217143	0.197522	175
3	0.373714	0.175497	175	0.194286	0.188678	175
5	0.373714	0.175497	175	0.194286	0.188678	175

	mean	std	count
length_pert	label			
1	0	14.071277	6.743926	940
1	11.114286	6.610560	175
3	0	22.126596	7.181945	940
1	17.782857	5.914014	175
5	0	25.192553	7.269947	940
1	20.291429	6.500282	175


dpos

		mean	std	count
length_pert	label			
1	0	15.873404	7.558641	940
1	13.788571	7.275837	175
3	0	25.031915	7.883540	940
1	21.234286	6.393870	175
5	0	28.454255	7.942889	940
1	23.942857	6.926307	175



DRMM
MSMARco

mean dist -- label =1 nqchange > 0

v1
mean	std	count
length_pert			
1	0.841288	0.147450	540
3	0.966052	0.064321	634
5	1.024848	0.041315	322




##### RANK DROP SUCCESS ####
WIKIQA
DRMM
PLEN    1       3       5
V1@1    100     100     100
V1@3    49.7    70.4    73.7
V1@5    25.8    45      48.8

PLEN    1       3       5
V2@1    92.5    62.4    70.4
V2@3    0       9.9     19.7
V2@5    0       2.3     8.9

PLEN    1       3       5
V3@1    100     100     100
V3@3    33.3    49.8    51.6
V3@5    15      24.9    26.8

V0@1
3    0.888393
5    1.236607

V0@3
3    0.566964
5    0.620536

v0@5
3    0.357143
5    0.383929

###DUET###

V0@1
3    1.000000
5    1.386935

V0@3
3    0.668342
5    0.708543

v0@5
3    0.422111
5    0.472362


V1@1
1    1.0
3    1.0
5    1.0

V1@3
1    0.512563
3    0.668342
5    0.668342

V1@5
1    0.266332
3    0.422111
5    0.467337

V2@1
1    0.648241
3    0.678392
5    0.683417

V2@3
1    0.005025
3    0.050251
5    0.090452

V2@5
3    0.005025
5    0.035176

V3@1
1    1.0
3    1.0
5    1.0

V3@3
1    0.497487
3    0.638191
5    0.643216

V3@5
1    0.251256
3    0.396985
5    0.402010


##KNRM##
V0@1

V0@3

v0@5


V1@1
1    1.0
3    1.0
5    1.0

V1@3
1    0.438679
3    0.599057
5    0.608491

V1@5
1    0.127358
3    0.297170
5    0.316038

V2@1
1    0.405660
3    0.773585
5    0.844340

V2@3
1    0.042453
3    0.231132
5    0.273585

V2@5
1    0.009434
3    0.051887
5    0.122642

V3@1
1    1.0
3    1.0
5    1.0

V3@3
1    0.424528
3    0.589623
5    0.617925

V3@5
1    0.132075
3    0.297170
5    0.316038

MSMARCO
DRMM
PLEN    1       3       5
V1@1    100     100     100
V1@3    32.9    75.9    90.1
V1@5    11.4    40.6    65.6

PLEN    1       3       5
V2@1    73.3    76.1    84.1
V2@3    1.7     8.3     15
V2@5    0.3     3.4     4.4

PLEN    1       3       5
V3@1    100     100     100
V3@3    15.7    38.9    49.2
V3@5    4       14.6    24.2

V0@1

V0@3

v0@5

DUET
V0@1

V0@3

v0@5


V1@1
1    1.0
3    1.0
5    1.0

V1@3
1    0.934066
3    1.000000
5    1.000000

V1@5
1    0.868132
3    0.967033
5    1.000000

V2@1
1    0.571429
3    0.571429
5    0.659341

V2@3
1    0.153846
3    0.285714
5    0.340659

V2@5
1    0.032967
3    0.098901
5    0.186813

V3@1
1    1.0
3    1.0
5    1.0

V3@3
1    0.934066
3    0.945055
5    0.978022

V3@5
1    0.813187
3    0.879121
5    0.934066


KNRM
V0@1

V0@3

v0@5


V1@1
length_pert
1    1.0
3    1.0
5    1.0

V1@3
1    0.971429
3    1.000000
5    1.000000

V1@5
1    0.897143
3    1.000000
5    1.000000

V2@1
1    0.891429
3    0.891429
5    0.942857

V2@3
1    0.520000
3    0.662857
5    0.742857

V2@5
1    0.451429
3    0.582857
5    0.668571

V3@1
1    1.0
3    1.0
5    1.0

V3@3
1    0.977143
3    1.000000
5    1.000000

V3@5
1    0.891429
3    1.000000
5    1.000000



\begin{comment}
% \small{$^+=pval<0.10$ and $^*=pval<0.05$ with 2 tailed ttest}}
\begin{comment}
\begin{table}[]
    \centering
    \begin{tabular}{ |c| c| c| }
 DRMM & Duet & KNRM \\ 
 cell4 & cell5 & cell6 \\  
 cell7 & cell8 & cell9    
    \end{tabular}
    \caption{Caption}
    \label{table:ranker_config}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c |c|c|c | }\hline
\textbf{Model} & \textbf{Fit}  & \multicolumn{3}{|c|}{WikiQA}   \\ \hline
\multirow{3}{*}{DRMM}  &v1& 0.977$\pm$0.003 & 0.927$\pm$0.005 & 0.878 $\pm$0.006  \\  
 &v2& 0.986$\pm$0.007 & 0.944$\pm$0.014 & 0.879$\pm$0.007\\
 &v3&0.977$\pm$0.003  & 0.953$\pm$0.004& 0.879$\pm$0.007\\ \hline
\multirow{3}{*}{KNRM} &v1& 0.978$\pm$0.004 & 0.930$\pm$0.005  & 	0.881$\pm$0.006  \\ 
 &v2& 0.989$\pm$0.007 & 0.948$\pm$0.009  & 0.911$\pm$0.006  \\ 
 &v3& 0.978$\pm$0.004 & 0.929$\pm$0.005  & 0.880$\pm$0.006 \\ \hline
 \multirow{3}{*}{Duet} &v1& 0.974$\pm$0.002 & 0.925$\pm$0.004  & 0.877$\pm$0.005  \\ 
 &v2& 0.986$\pm$0.007 & 0.947$\pm$0.010  & 0.913$\pm$0.005   \\ 
 &v3& 0.974$\pm$0.002 & 0.926$\pm$0.004  & 0.877$\pm$0.006 \\ \hline
    \end{tabular}
    \caption{Emb sim b/w perturbed \& original WikiQA ans}
    \label{table:wikiqa_cosine}
\end{table}

\end{comment}

